On the Performance of Reed-Muller Codes Over $(d,\infty)$-RLL Input-Constrained BMS Channels

This paper considers the input-constrained binary memoryless symmetric (BMS) channel, without feedback. The channel input sequence respects the $(d,\infty)$-runlength limited (RLL) constraint, which mandates that any pair of successive $1$s be separated by at least $d$ $0$s. We consider the problem of designing explicit codes for such channels. In particular, we work with the Reed-Muller (RM) family of codes, which were shown by Reeves and Pfister (2021) to achieve the capacity of any unconstrained BMS channel, under bit-MAP decoding. We show that it is possible to pick $(d,\infty)$-RLL subcodes of a capacity-achieving (over the unconstrained BMS channel) sequence of RM codes such that the subcodes achieve, under bit-MAP decoding, rates of $C\cdot{2^{-\left \lceil \log_2(d+1)\right \rceil}}$, where $C$ is the capacity of the BMS channel. Finally, we also introduce techniques for upper bounding the rate of any $(1,\infty)$-RLL subcode of a specific capacity-achieving sequence of RM codes.

==> BCJR_invar.tex <==
\label{subsec:BCJR_invar}

Given the $Q$-graph, $\mathscr{G}_Q^{(d)}$, for the $(d,\infty)$-RLL input constrained BEC, we call its corresponding $(S,Q)$ graph, $\mathscr{G}_{SQ}^{(d)}$, which is constructed following the description in definition \ref{def:SQ_graph}, with the presentation of channel states given in figure \ref{fig:d_inf_constraint}. 


%We note that our family of $(S,Q)$-graphs  possesses the following interesting property:
%
%\begin{proposition}\label{prop:lp}
%	In the setting of the $(d,\infty)$-RLL input-constrained BEC, for the $(S,Q)$-graphs, $\mathscr{G}_{SQ}^{(d)}$, we have that 
%	\begin{equation*}
%	\max_{\{{P}(x|s,v)\}} P(X=1)\leq \frac{1}{d+1},
%	\end{equation*}
%	where the maximum is taken over all input distributions, $\left({P}(\cdot|s,v): s\in \mathscr{S},\ v\in \mathscr{V}^{(d)}\right)$ such that the resulting Markov chain on $\mathscr{S}\times \mathscr{V}^{(d)}$ has a unique stationary distribution.
%\end{proposition}
%
%We prove Proposition \ref{prop:lp} by casting the maximization problem as a linear program (LP). We then use the weak duality theorem for LPs (see, for example, \cite{boyd}) to find a feasible point of the corresponding dual LP, the objective value at which serves as an upper bound for our maximization problem. The proof is dealt with in Appendix C.

In this subsection, we construct a BCJR-invariant input distribution, $\left(\left(\tilde{P}(x|s,v):x\in \mathscr{X}\right): (s,v)\in \mathscr{S}\times \mathscr{V}^{(d)}\right)$. In tandem, we will also identify the conditional distribution, $\left(\tilde{\pi}(s|v):s\in \mathscr{S}\right)$, for each $v\in \mathscr{V}^{(d)}$, where $\left(\tilde{\pi}(s,v):s\in \mathscr{S},\ v\in \mathscr{V}^{(d)}\right)$ is the stationary distribution on the nodes of $\mathscr{G}_{SQ}^{(d)}$
%, and $\tilde{\pi}(v) = \sum_{s\in \mathscr{S}}\tilde{\pi}(s,v)$.

%Before we do so, it will be useful to put down some additional notation. Now, for $\mathbf{q}\in \mathscr{V}^{(d)}$, let $(k_1^{\mathbf{q}},k_2^{\mathbf{q}},\ldots,k_{d+1}^{\mathbf{q}})$ denote the runlength sequence of $0$s and $?$s, in $\mathbf{q}$, defined as follows:

%If $\mathbf{q}$ begins with a run of $\ell$ $0$s, for $\ell \geq 1$, then $k_1^{\mathbf{q}} = \ell$; otherwise, $k_1^{\mathbf{q}} = 0$. Further, $k_2^{\mathbf{q}}$ is the length of the run of $?$s after the first run (if any) of $0$s; $k_3^{\mathbf{q}}$ is the length of the (second) run of $0$s after the first run of $?$s, and so on. 

%Note that $k_{2i-1}^{\mathbf{q}}$ records the length of a run of $0$s and $k_{2i}^{\mathbf{q}}$ records the length of a run of $?$s, for $i\geq 1$. Also, $k_{d+1}^{\mathbf{q}}\neq 0$ if, and only if, $\mathbf{q}$ is such that $q_{2i-1}=?$ and $q_{2i}=0$, for $i\geq 1$. Observe that $\sum_{i=1}^{d+1}k_i^{\mathbf{q}} = d$ and $k_i^{\mathbf{q}}\geq 0$, for all $i\in [d+1]$. We shall henceforth omit the superscript $\mathbf{q}$ since it will be apparent from the context.

Since our input distribution %$\left(\tilde{P}(\cdot|s,v):s\in \mathscr{S},\ v\in \mathscr{V}^{(d)}\right)$,
must respect the $(d,\infty)$ input constraint, we need that $\tilde{P}(1|s,v)=0$, for $s\in \{0,1,\ldots,d-1\}$, and we hence need only specify $\tilde{P}(1|d,v)$, for each $v\in \mathscr{V}^{(d)}$, to completely determine the input distribution.

To this end, we first associate with every node $v\in \mathscr{V}^{(d)}$, a probability vector, $\boldsymbol{\theta}_v:=\left(\theta_v(s):s\in \mathscr{S}\right)$, of length $d+1$. 
%The vector $\boldsymbol{\theta}_v$ is a proxy for $\left(\tilde{\pi}(s|v):s\in \mathscr{S}\right)$ for a suitably defined input distribution.

We set $\boldsymbol{\theta}_{Q_i} = \mathbf{e}_{i}^{d}$, for $i\in [0:d]$. Further, in compliance with the $(d,\infty)$-RLL input constraint, we set $a_{Q_i}:=\tilde{P}(1|d,Q_i) = 0$, for $i\neq d$. Let us pick $a := \tilde{P}(1|d,Q_d)$, such that $a\leq \frac{1}{d+1}$. The reason for the restriction of $a$ to the interval $[0,\frac{1}{d+1}]$ will be made clear in Lemma \ref{lemma:domain}. 
%We shall, for conciseness of notation, represent $a_{Q_d}$ as $a$.

Now, for $\mathbf{q} = (w_{0},w_{1},\ldots,w_{d-1})\in \mathscr{V}^{(d)}_{\text{DB}}$, we define an accompanying vector $\boldsymbol{\beta}=(\beta_{0},\beta_{1},\ldots,\beta_{d-1})$, with\\ $\beta_s := |\{i\in [0:s-1]:w_i=0\}|$. In words, $\beta_s$ is the number of $0$s that appear strictly to the left of position $s$ in the $d$-tuple corresponding to $\mathbf{q}$. We then define $\boldsymbol{\theta}_{\mathbf{q}}$ as follows:

For $0\leq s\leq d-1$,
\begin{equation}\label{eq:theta_even}
{\theta}_{\mathbf{q}}(s) = 
\begin{cases}
0, & \text{ if } w_s=0,\\
\frac{a}{(1-a)^{\beta_s}}, & \text{ if }  w_s=\ ?,
\end{cases}
\end{equation}
and $\theta_{\mathbf{q}}(d) = 1-\sum_{s=0}^{d-1}\theta_{\mathbf{q}}(s)$. It is clear from our definition that $\boldsymbol{\theta}_{Q_d} = \mathbf{e}_{d}^{d}$, where $Q_d = (0,0,\ldots,0)\in \mathscr{V}_{\text{DB}}^{(d)}$.

%If $d$ is odd, for $\mathbf{q} \in \mathscr{V}_{\text{DB}}^{(d)}$, we set
%\begin{equation}\label{eq:theta_odd}
%\theta_{\mathbf{q}}(s) = 
%\begin{cases}
%a, \ s\in [0:k_{d+1}-1],\\
%0, \ s\in [k_{d+1}:k_{d+1}+k_d-1],\\
%\frac{a}{(\bar{a})^{k_d}}, \ s\in [k_{d+1}+k_d:\sum\limits_{i\geq {d-1}}k_i -1],\\
%0, \ s\in [\sum\limits_{i\geq {d-1}}k_i:\sum\limits_{i\geq {d-2}}k_i-1],\\
%\quad \vdots\\
%\frac{a}{(\bar{a})^{\sum\limits_{i\geq 3: i\ \text{odd}}k_i}}, \ s\in [\sum\limits_{i\geq {3}}k_i:\sum\limits_{i\geq {2}}k_i],\\
%0, \ s\in [\sum\limits_{i\geq {2}}k_i:d-1],
%\end{cases}
%\end{equation}
%and $\theta_{\mathbf{q}}(d) = 1-\sum_{i=1}^{d-1}\theta_{\mathbf{q}}(i)$.

Finally, for $\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}$, we let $a_{\mathbf{q}}:= \tilde{P}(1|d,\mathbf{q}) = \frac{a}{\theta_{\mathbf{q}}(d)}$. In order for $a_{\mathbf{q}}$ to be a valid probability, it must lie in $[0,1]$, a sufficient condition for which is provided by Lemma \ref{lemma:domain} below.

\begin{lemma}\label{lemma:domain}
	For $a\in [0,\frac{1}{d+1}]$, $a_{\mathbf{q}}\in [0,1]$, for $\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}$ .
\end{lemma}

%The proof of this lemma is taken up in  Appendix A.
We refer the reader to \cite{fv} for the proof of the lemma above.
\begin{remark}
%Note that this procedure determines the vector $\left(a_v:v\in \mathscr{V}^{(d)}\right)$, thereby specifying the entire input distribution $\left(\tilde{P}(\cdot|s,v):s\in \mathscr{S},\ v\in \mathscr{V}^{(d)}\right)$.

Our input distribution is aperiodic for $a<\frac{1}{d+1}$ and $\epsilon\neq 1$, as then there exists a self-loop of positive probability, $\bar{a}\bar{\epsilon}$, from the node $(d,Q_d)$ to itself, in $\mathscr{G}_{SQ}^{(d)}$. The feedback capacity at $\epsilon=1$ is well-known to be $C^{\text{fb}}(1) = 0$, and we safely assume, going forward, that $\epsilon\neq 1$.
\end{remark}

%\begin{figure*}[t]
%	\centering
%	\subfloat[]{\includegraphics[width=0.2\linewidth]{1_inf.png}\label{fig:Q_1}}
%	\hfill
%	\subfloat[]{\includegraphics[width=0.4\linewidth]{2_inf.png}\label{fig:Q_2}}
%	\caption{The $Q$-graphs $\mathscr{G}^{(1)}_Q$ and $\mathscr{G}^{(2)}_Q$ are shown above in (a) and (b), respectively. Note that the nodes in the de Bruijn components are labelled by $d$-tuples, with $Q_1 = 0$, in $\mathscr{G}^{(1)}_Q$, and $Q_2 = (0,0)$, in $\mathscr{G}^{(2)}_Q$. The parallel edges defined are here represented as a single edge with the label $(0,?)$, according to \eqref{eq:label}.}
%\end{figure*}
%\begin{figure}[t]
%	\centering
%	\includegraphics[scale=0.5]{2_inf_mod.png}
%	\caption{The $Q$-graph $\mathscr{G}^{(2)}_Q$ is shown above. Note that the nodes in the de Bruijn components are labelled by $d$-tuples, with $Q_2 = (0,0)$. The parallel edges defined are here represented as a single edge with the label $(0,?)$, according to \eqref{eq:label}.}
%	\label{fig:Q_2}
%\end{figure}
%Before we set out to prove that the aperiodic input distribution $\tilde{P}$ is indeed BCJR invariant, we shall introduce one other piece of notation. For the function $B_s: \Delta(d)\times \mathscr{Y} \rightarrow \Delta(d)$ defined in equation \eqref{eq:bs}, we define the vector $\mathbf{B}(\mathbf{\theta_v},y)$ to be $\left(B_s(\mathbf{\theta_v},y): s\in \mathscr{S}, s\neq d\right)$, for $v\in \mathscr{V}^{(d)}$. For the $(d,\infty)$-RLL input constrained BEC with the input distribution $\tilde{P}$, we can write down $\mathbf{B}(\mathbf{\theta_v},y)$ explicitly. For $v\in \mathscr{V}_{\text{DB}}^{(d)}$,

Before we prove that the aperiodic input distribution $\tilde{P}$ is indeed BCJR-invariant, we note that for all $s\in \mathscr{S}$ and $v\in \mathscr{V}^{(d)}$, the value $B_s(\boldsymbol{\theta}_v,y)$ (see equation \eqref{eq:bs}) can be computed explicitly for the $(d,\infty)$-RLL input constrained BEC with the input distribution $\tilde{P}$. 
%\begin{equation*}
%\mathbf{B}(\mathbf{\theta_v},y) = \begin{cases}
%\left[0,\frac{\theta_{\mathbf{q}}(0)}{1-a_\mathbf{q}\theta_{\mathbf{q}}(d)},\frac{\theta_{\mathbf{q}}(1)}{1-a_\mathbf{q}\theta_{\mathbf{q}}(d)},\ldots,\frac{\theta_{\mathbf{q}}(d-2)}{1-a_\mathbf{q}\theta_{\mathbf{q}}(d)}\right], \ y=0,\\
%\left[a_\mathbf{q}\theta_{\mathbf{q}}(d),\theta_{\mathbf{q}}(0),\theta_{\mathbf{q}}(1),\ldots,\theta_{\mathbf{q}}(d-2)\right], \ y=?,\\
%[1,0,0,\ldots,0], \ y=1,
%\end{cases}
%\end{equation*}
%
For $0\leq s\leq d-1$, and for $\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}$, it holds that
\begin{equation}\label{eq:Bs0}
B_s(\boldsymbol{\theta}_\mathbf{q},y) = 
\begin{cases}
0, & \text{ if } s=0,\ y=0\\
\frac{\theta_{\mathbf{q}}(s-1)}{1-a_\mathbf{q}\theta_{\mathbf{q}}(d)} = \frac{\theta_{\mathbf{q}}(0)}{1-a}, & \text{ if } 1\leq s \leq d-1, \ y=0\\
a_\mathbf{q}\theta_{\mathbf{q}}(d) = a & \text{ if } s=0, \ y=?\\
\theta_{\mathbf{q}}(s-1), & \text{ if } 1\leq s \leq d-1, \ y=?\\
1, & \text{ if } s=0, \ y=1\\
0, & \text{ if } 1\leq s \leq d-1, \ y=1,
\end{cases}
\end{equation}
with $B_d(\boldsymbol{\theta}_\mathbf{q},y) = 1 - \sum_{s=0}^{d-1}B_s(\boldsymbol{\theta}_\mathbf{q},y)$, for $y\in \{0,?,1\}$. Note that the vector $\left(B_s(\boldsymbol{\theta}_\mathbf{q},1): s\in \mathscr{S}\right)$ is equal to $\mathbf{e}_0^{d}$.
%which results in
%\begin{equation}\label{eq:bs_BEC}
%\mathbf{B}(\mathbf{\theta_v},y) = 
%\begin{cases}
%\left[0,\frac{\theta_{\mathbf{q}}(0)}{1-a},\frac{\theta_{\mathbf{q}}(1)}{1-a},\ldots,\frac{\theta_{\mathbf{q}}(d-2)}{1-a}\right], \ y=0,\\
%\left[a,\theta_{\mathbf{q}}(0),\theta_{\mathbf{q}}(1),\ldots,\theta_{\mathbf{q}}(d-2)\right], \ y=?,\\
%[1,0,0,\ldots,0], \ y=1,
%\end{cases}
%\end{equation}
%since $a_\mathbf{q}\theta_{\mathbf{q}}(d)=a$.

Further, if $v=Q_i$, for some $i\in [0:d-1]$, it holds that
\begin{equation}\label{eq:BsQ}
\left(B_s(\boldsymbol{\theta}_v,y): s\in \mathscr{S}\right) = \mathbf{e}_{i+1}^{d},
\end{equation}
for $y\in \{0,?\}$.
%\begin{equation}\label{eq:bs_BEC_2}
%\mathbf{B}(\mathbf{\theta_v},y) = \mathbf{e}_{i+1}^{d},\ \text{for}\ y\in \{0,?\}.
%\end{equation} 
We now note that the following lemma holds:

\begin{lemma}\label{lemma:bcjr}
	The set of probability vectors $\left(\boldsymbol{\theta}_{v}: v\in \mathscr{V}^{(d)}\right)$ along with the input distribution $\left(\tilde{P}(\cdot|s,v):s\in \mathscr{S},\ v\in \mathscr{V}^{(d)}\right)$ satisfies
	\begin{equation}\label{eq:bs_valid}
	\theta_{v^+}(s^+) = B_{s^+}(\boldsymbol{\theta}_v,y),
	\end{equation}
	for every $(s^+,v,y)\in \mathscr{S}\times \mathscr{V}^{(d)}\times \mathscr{Y}$, where $v^+ = \Phi(v,y)$, with $\Phi:\mathscr{V}^{(d)}\times \mathscr{Y}\rightarrow \mathscr{V}^{(d)}$ is the $Q$-node update function.
\end{lemma}
\begin{proof}
	If $v=Q_i$, for some $i\in [0:d-1]$, then, it follows from equation \eqref{eq:BsQ} that 	
	$\mathbf{e}_{i+1}^{d}=\left(B_s(\boldsymbol{\theta}_{Q_i},y):s\in \mathscr{S}\right)
	$ which, in turn, is equal to  $\boldsymbol{\theta}_{Q_{i+1}}$,	
	for $y\in \{0,?\}$. Equation \eqref{eq:bs_valid} then follows by noting that $\Phi(Q_i,y) = Q_{i+1}$, for $y\in \{0,?\}$.
	
	Now, for $\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}$, when $y=1$, we see from equation \eqref{eq:Bs0} that	
	$\mathbf{e}_{0}^{d}=\left(B_s(\boldsymbol{\theta}_{v},1):s\in \mathscr{S}\right)$, which is equal to $\boldsymbol{\theta}_{Q_{0}}$.
	Since $\Phi(v,1) = Q_{0}$, it follows that equation \eqref{eq:bs_valid} holds.
	
	Now, let $\mathbf{q} = (w_{0},w_{1},\ldots,w_{d-1})\in \mathscr{V}_{\text{DB}}^{(d)}$. Then, since $\Phi(\mathbf{q},0) = (0,w_{0},w_{1},\ldots,w_{d-1}))=:\mathbf{q}_0^+$, and $\Phi(\mathbf{q},?) = (?,w_{0},w_{1},\ldots,w_{d-1})=:\mathbf{q}_?^+$,  we see from equations \eqref{eq:theta_even} and \eqref{eq:Bs0} that $\left(B_s(\boldsymbol{\theta}_\mathbf{q},0):s\in\mathscr{S}\right) = \boldsymbol{\theta}_{\mathbf{q}^+_0}$ and $\left(B_s(\boldsymbol{\theta}_\mathbf{q},?):s\in\mathscr{S}\right) = \boldsymbol{\theta}_{\mathbf{q}^+_?}$. Thus, equation \eqref{eq:bs_valid} holds in this case too.	
\end{proof}
We now define the joint distribution, $\theta(s,v):=\theta_v(s)\tilde{\pi}(v)$, where $\left(\tilde{\pi}(v):v\in \mathscr{V}^{(d)}\right)$ is the stationary distribution on the nodes of $\mathscr{G}_Q^{(d)}$ induced by $\tilde{P}$. From Lemma \ref{lemma:bcjr} and from the lemma below, we get that $\tilde{P}$ is BCJR-invariant.

\begin{lemma}\label{lemma:stat_dist}
	It holds that $\theta(s,v) = \tilde{\pi}(s,v)$, for all $s\in \mathscr{S}$ and $v\in \mathscr{V}^{(d)}$.
\end{lemma}
\begin{proof}
	Fix an $s^+ \in \mathscr{S}$, and a $v^{+}\in \mathscr{V}^{(d)}$. Now,
	\begin{align*}
	&\sum\limits_{s,v,x,y}\theta(s,v)P(x|s,v)P(y|x)\mathds{1}\{s^+=f(x,s)\}\mathds{1}\{v^+=\Phi(v,y)\}\\
	&= \sum\limits_{v,y}\tilde{\pi}(v)\mathds{1}\{v^+=\Phi(v,y)\}\sum\limits_{x,s}\theta_v(s)P(x|s,v)P(y|x)\times\\
	&\quad \quad \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad \mathds{1}\{s^+=f(x,s)\}\\
	&\stackrel{(a)}{=}\theta_{v^+}(s^+)\sum\limits_{v,y}\tilde{\pi}(v)P(y|v)\mathds{1}\{v^+=\Phi(v,y)\}\\
	&=\theta_{v^+}(s^+)\tilde{\pi}(v^+) = \theta(s^+,v^+),
	\end{align*}
	where (a) follows from Lemma \ref{lemma:bcjr}, since $\theta_{v^+}(s^+)P(y|q)=\sum\limits_{x,s}\theta_v(s)P(x|s,v)P(y|x)\mathds{1}\{s^+=f(x,s)\}$. Since this holds for all $(s^+,v^+) \in \mathscr{S}\times \mathscr{Y}$, it follows that $\theta(s^+,v^+) = \tilde{\pi}(s^+,v^+)$.
\end{proof}
The lemma above implies that $\boldsymbol{\theta}_v = \tilde{\pi}(\cdot|v)$, and using Lemma \ref{lemma:bcjr}, we can conclude that $\tilde{P}$ is BCJR-invariant.
\begin{remark}
	It can be shown that for a fixed value of $a$, there is a unique BCJR-invariant input distribution on $\mathscr{G}_{SQ}^{(d)}$. 
	%In particular, this means that for a fixed value of $a$, the probability\\ $P(Y=1|\mathbf{q}) = a\epsilon$, for all $\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}$.
\end{remark}

==> Proof_UB.tex <==
\label{sec:proof_UB}
\begin{proof}
We shall compute the upper bound expression in theorem \ref{thm:UB} by considering the family of $Q$-graphs, $\mathcal{J}:=\{\hat{\mathscr{G}}_Q^{(d)}: d\in \mathbb{N}\}$, where $\hat{\mathscr{G}}_Q^{(d)}$ is shown in figure \ref{fig:G_hat} for some fixed $d$. Let $\hat{\mathscr{G}}_{SQ}^{(d)}$ denote the $(S,Q)$-graph corresponding to $\hat{\mathscr{G}}_Q^{(d)}$. 

\begin{figure*}[t]
	\centering
	\includegraphics[width=0.5\textwidth]{UB_Q.png}
	\caption{The $Q$-graph, $\hat{\mathscr{G}}_Q^{(d)}$. The labels on the edges denote outputs.}
	\label{fig:G_hat}
\end{figure*}

It can be shown that the single closed communicating class in $\hat{\mathscr{G}}_{SQ}^{(d)}$ is precisely the collection $\{(i,\hat{Q}_i): i\in [0:d-1]\}\cup \{(s,\hat{Q}_d):s\in [0:d]\}$ of nodes. Further, since the inputs are constrained, it holds that $P(X=1|S=s,Q=\hat{q}) = 0$, for all $(s,\hat{q}) \neq (d,\hat{Q}_d)$, with $(s,\hat{q})$ in the closed class. Therefore, the matrix of conditional input distributions, $[P(x|s,\hat{q})]$, can be parameterized by a single parameter, $p:=P(X=1|S=d,Q=\hat{Q}_d)$.

A simple computation then reveals that the stationary distribution of nodes in the closed communicating class obey:
\begin{align*}
\pi(s,\hat{Q}_s) &= \frac{p\bar{\epsilon}}{1+dp}, \ s\in [0:d-1],\\
\pi(s,\hat{Q}_d) &= \frac{p\epsilon}{1+dp}, \ s\in [0:d-1], \\
\pi(d,\hat{Q}_d) &= \frac{1}{1+dp}.
\end{align*}
Further, it holds that the conditional probability,

\begin{align*}
P(Y=1|\hat{Q}_d) &= P(Y=1,X=1,S=d|\hat{Q}_d)\\
&=p\bar{\epsilon}\frac{\pi(d,\hat{Q}_d)}{\sum_{s=0}^{d}\pi(s,\hat{Q}_d)}\\
&= \frac{p\bar{\epsilon}}{1+dp\epsilon}.
\end{align*}

Then, by Theorem \ref{thm:UB}, it holds that
\begin{align*}
C_{(d,\infty)}^{\text{fb}} &\leq \sup_{P(x|s,q)\in \Omega} I(X;Y|Q)\\
&= \sup_{P(x|s,q)\in \Omega} H(Y|Q) - h_b(\epsilon)\\
&\stackrel{(a)}{=} \max_{p\in [0,1]} \bar{\epsilon}\left(\sum_{s=0}^{d}\pi(s,\hat{Q}_d)\right)h_b\left(\frac{p}{1+dp\epsilon}\right)\\
&= \max_{p\in [0,1]} \frac{\bar{\epsilon}(1+dp\epsilon)}{1+dp}h_b\left(\frac{p}{1+dp\epsilon}\right)\\
&\stackrel{(b)}{=} \max_{\delta \in [0,\frac{1}{1+d\epsilon}]} R(\delta),
\end{align*}
where, in (a), we have used the identity that $H(a\bar{c},\bar{a}\bar{c},c) = h_b(c)+\bar{c}h_b(a)$, for all $a,c \in [0,1]$, and (b) follows by changing the variable used in the maximization to $\delta:= \frac{p}{1+dp\epsilon}$.

Now, we note that if $\epsilon^{\star}$ satisfies the equation
\[
(d\epsilon)^{\left(\frac{1}{1-\epsilon}+d\right)} = (1+d\epsilon)^d,
\]
then, the derivative evaluated at $\frac{1}{1+d\epsilon^{\star}}$,  $R^{\prime}\left(\frac{1}{1+d\epsilon^{\star}}\right)$, is equal to $0$. Further, from the proof of Corollaries \ref{coroll} in Appendix B, we observe that $R^{\prime}(\delta)$ is strictly decreasing in $\delta$, for $\delta\in [0,1]$. Hence, it follows that for $\epsilon>\epsilon^{\star}$, the derivative, $R^{\prime}\left(\frac{1}{1+d\epsilon}\right)>0$, with $R^{\prime}(0^+)>0$. 

Therefore, the non-causal capacity, which is a maximum over $[0,1]$ of $R(\delta)$, is strictly larger than the upper bound in Proposition \ref{lemma:UB}, for $\epsilon>\epsilon^{\star}$.
\end{proof}

==> Proof_main.tex <==
\label{sec:proof_thm}

\begin{proof}
For the $(d,\infty)$-RLL input-constrained BEC under the BCJR-invariant input distribution $\tilde{P}$ defined in subsection \ref{subsec:BCJR_invar}, we have that
\begin{align*}
I(X;Y|Q) &\stackrel{(a)}{=} H(Y|Q) - h_b(\epsilon)\\
&\stackrel{(b)}{=} \bar{\epsilon}\sum_{v\in \mathscr{V}^{(d)}}\tilde{\pi}(v)h_b(P(X=1|v)) + h_b(\epsilon)- h_b(\epsilon)\\
&\stackrel{(c)}{=} \bar{\epsilon}\sum_{\mathbf{q}\in \mathscr{V}^{(d)}_{\text{DB}}}\tilde{\pi}(\mathbf{q})h_b(P(X=1|\mathbf{q}))\\
&\stackrel{(d)}{=}\bar{\epsilon}h_b(a)\sum_{\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}}\tilde{\pi}(\mathbf{q}).
\end{align*}
where (a) follows from the fact that $H(Y|X,Q) = H(Y|X) = h_b(\epsilon)$, and (b) from the fact that $P(Y=?|v) = \epsilon$, for all $v\in \mathscr{V}^{(d)}$, with $P(Y=1|v) = \bar{\epsilon}P(X=1|v)$. We additionally use  the identity that $H(a\bar{c},\bar{a}\bar{c},c) = h_b(c)+\bar{c}h_b(a)$, for all $a,c \in [0,1]$. Further, (c) holds since $P(X=1|Q_i) = 0$, for $i\in [0:d-1]$. To obtain the equality (d), note that for any $\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}$, $P(X=1|\mathbf{q}) = \tilde{\pi}(d|\mathbf{q})a_\mathbf{q}$. Hence, from Lemma \ref{lemma:stat_dist}, it follows that that $P(X=1|\mathbf{q}) = a$.

%Now, since for any $\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}$, $P(X=1|\mathbf{q}) = \tilde{\pi}(d|\mathbf{q})a_\mathbf{q}$, we get from Lemma \ref{lemma:stat_dist} that $P(X=1|\mathbf{q}) = a$. Hence, it follows that
%
%\begin{equation}\label{eq:I_eval}
%I(X;Y|Q) = \bar{\epsilon}h_b(a)\sum_{\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}}\tilde{\pi}(\mathbf{q}).
%\end{equation}
Further, it is true that
\begin{align}\label{eq:stat_q}
1 &= \sum_{\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}}\tilde{\pi}(\mathbf{q}) + \sum_{i=0}^{d-1}\tilde{\pi}(Q_i) \notag\\
&= \sum_{\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}}\tilde{\pi}(\mathbf{q}) + d\tilde{\pi}(Q_0) \notag\\
&= (1+da\bar{\epsilon})\sum_{\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}}\tilde{\pi}(\mathbf{q}),
\end{align}
where the penultimate equality holds since $\tilde{\pi}(Q_0) = \tilde{\pi}(Q_i)$, for all $i\in [d-1]$. The last equality follows from the observation that $\tilde{\pi}(Q_0) = \sum_{\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}}\tilde{\pi}(\mathbf{q})P(Y=1|\mathbf{q}) = \bar{\epsilon}a\sum_{\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}}\tilde{\pi}(\mathbf{q})$.

Plugging \eqref{eq:stat_q} back into equation (d), we obtain that $I(X;Y|Q) = \frac{h_b(a)}{da+\frac{1}{1-\epsilon}}$, and taking a maximum over all \\$a\in [0,\frac{1}{d+1}]$, we get the required result.
\end{proof}



==> Q-construction.tex <==
\label{sec:Q_const}
%We shall henceforth consider $\mathscr{S} = \{0,1,\ldots,d\}$ to be the state alphabet, for the $(d,\infty)$-RLL input constrained BEC.
%
%
In this section, we shall construct a family of $Q$-graphs, indexed by $d$, and identify a BCJR-invariant input distribution on the $(S,Q)$-graph corresponding to each $Q$-graph in the family.

\subsection{Construction of Q-graphs}
\input{Q-graph_fly.tex}

\subsection{Construction of a BCJR-invariant input distribution}
\input{BCJR_invar.tex}

==> Q-graph_fly.tex <==
%First, we recall the definition of a De Bruijn graph.
%
%\begin{definition}
%	Given an alphabet $\Sigma = \{w_1,w_2,\ldots,w_m\}$, a $k$-dimensional De Bruijn graph $\mathscr{G}_{\text{DB}}^{(k)} = (\mathscr{V}_{\text{DB}}^{(k)},\mathscr{E}_{\text{DB}}^{(k)},\mathscr{L}_{\text{DB}}^{(k)})$ over $\Sigma$ is a labelled, directed graph with vertex set $\mathscr{V}_{\text{DB}}^{(k)}$, edge set $\mathscr{E}_{\text{DB}}^{(k)}$, and a labelling function $\mathscr{L}_{\text{DB}}^{(k)}: \mathscr{E}_{\text{DB}}^{(k)}\rightarrow \Sigma$. Each vertex $v\in \mathscr{V}$ can be uniquely identified by a $k$-tuple over $\Sigma$, i.e., each vertex in $\mathscr{V}_{\text{DB}}^{(k)}$ can alternatively be written as $\mathbf{v} = (w_1^v,w_2^v,\ldots,w_k^v)$, where $w^v_i \in \Sigma$, for $i\in [k]$. Note that there are $m^k$ vertices in total.
%	
%	The edge set 	
%	\begin{align*}
%	\mathscr{E}_{\text{DB}}^{(k)} = \lbrace\mathbf{e}:\mathbf{e} = &\left((w_1^i,w_2^i\ldots,w_k^i),(w_2^i,w_3^i,\ldots,w_k^i,w)\right),\\
%	& \text{ for some $w_1^i,\ldots,w_k^i,w \in \Sigma$}\rbrace.
%	\end{align*}
%	
%	Further, for any edge \\$\mathbf{e} = \left((w_1^i,w_2^i\ldots,w_k^i),(w_2^i,w_3^i,\ldots,w_k^i,w)\right)$, we write \\ $\mathscr{L}(\mathbf{e}) = w$.
%\end{definition}
With each value of $d$ corresponding to the $(d,\infty)$-RLL input-constrained BEC, we associate a $Q$-graph, $\mathscr{G}_{Q}^{(d)} = (\mathscr{V}^{(d)},\mathscr{E}^{(d)},\mathscr{L}^{(d)})$, with vertex set $\mathscr{V}^{(d)}$, edge multi-set $\mathscr{E}^{(d)}$, and a labelling function $\mathscr{L}^{(d)}: \mathscr{E}^{(d)}\rightarrow \{0,?,1\}$.

We write $\mathscr{V}^{(d)} = \mathscr{V}_{\text{DB}}^{(d)} \cup \{Q_0, Q_1,\ldots,Q_{d-1}\}$, where each vertex in $\mathscr{V}_{\text{DB}}^{(d)}$ is uniquely identified by a $d$-tuple over $\{0,?\}$, i.e., each vertex in $\mathscr{V}_{\text{DB}}^{(d)}$ can be written as $\mathbf{q} = (w_{0}^q,w_{1}^q,\ldots,w_{d-1}^q)$, where $w^q_i \in \{0,?\}$, for $i\in \{0,1,\ldots,d-1\}$. In what follows, we suppress the superscript $q$, as it will be clear from the context. Note that there are $2^d$ vertices in $\mathscr{V}_{\text{DB}}^{(d)}$. We denote by $Q_d$, the vertex $(0,0,\ldots,0)\in \mathscr{V}_{\text{DB}}^{(d)}$.\footnote{The subscript ``DB'' indicates that the subgraph $\mathscr{G}_{\text{DB}}^{(d)} = (\mathscr{V}_{\text{DB}}^{(d)},\mathscr{E}_{\text{DB}}^{(d)},\mathscr{L}_{\text{DB}}^{(d)})$, of $\mathscr{G}_{Q}^{(d)}$, is a de Bruijn graph of order $d$, on $\{0,?\}$ symbols.}


We now construct the edge multi-set, $\mathscr{E}^{(d)}$. Firstly, for vertices in $\mathscr{V}_{\text{DB}}^{(d)}$, we define the set $\mathscr{E}_{\text{DB}}^{(d)}$ to consist of all edges $\mathbf{e} = \left((w_{0},w_{1}\ldots,w_{d-1}),(w,w_{0},w_1,\ldots,w_{d-2})\right)$, for $(w_{0},w_1\ldots,w_{d-1}), \ (w,w_{0},\ldots,w_{d-2}) \in \mathscr{V}_{\text{DB}}^{(d)}$. 
%\begin{align*}
%	\mathscr{E}_{\text{DB}}^{(d)} = & \lbrace\mathbf{e}:\mathbf{e} = \left((w_{0},w_{1}\ldots,w_{d-1}),(w,w_{0},w_1,\ldots,w_{d-2})\right),\\
%	& \ \ \ \ \ \text{ for }(w_{0},w_1\ldots,w_{d-1}), \ (w,w_{0},\ldots,w_{d-2}) \in \mathscr{V}_{\text{DB}}^{(d)} \rbrace.
%\end{align*}
%
Further, for any edge $\mathbf{e} = \bigl((w_{0},w_{1}\ldots,w_{d-1})$, $(w,w_{0},w_{1},\ldots,w_{d-2})\bigr)$, we define the labelling function $\mathscr{L}_{\text{DB}}^{(d)}: \mathscr{E}_{\text{DB}}^{(d)}\rightarrow \{0,?\}$ such that $\mathscr{L}_{\text{DB}}^{(d)}(\mathbf{e}) = w$.

%In this discussion, we shall focus on $d$-dimensional De Bruijn graphs, $\mathscr{G}_{\text{DB}}^{(d)}$, over $\Sigma = \{0,?\}$. By the definition above, this is a graph with $2^d$ vertices, each identified by a unique $d$-tuple consisting of $0,?$ symbols. Let us denote by $Q_d$, the vertex $(0,0,\ldots,0)\in \mathscr{V}_{\text{DB}}^{(d)}$.

%We construct the $Q$-graph, $\mathscr{G}_Q^{(d)} = (\mathscr{V}^{(d)},\mathscr{E}^{(d)},\mathscr{L}^{(d)})$, where $\mathscr{E}^{(d)}$ is now taken to be a multi-set, by first adding $d$ additional vertices, $Q_0,Q_1,\ldots, Q_{d-1}$, to $\mathscr{V}_{\text{DB}}^{(d)}$. Hence, $\mathscr{V}^{(d)} = \mathscr{V}_{\text{DB}}^{(d)} \cup \{Q_0,\ldots,Q_{d-1}\}$.

The edge set, $\mathscr{E}^{(d)}$, is constructed by adding to the set $\mathscr{E}_{\text{DB}}^{(d)}$, the edges $(\mathbf{q},Q_0)$, for $\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}$, and, corresponding to each $Q_i$, $i\in [0:d-1]$, two edges, $\mathbf{e}^{Q_i}_1$ and $\mathbf{e}^{Q_i}_2$, from $Q_i$ to $Q_{i+1}$. %Note that the $Q$-graph, $\mathscr{G}_Q^{(d)}$, has parallel edges. %which are precisely the edges from $Q_i$ to $Q_{i+1}$, for $i\in [0:d-1]$.

%\begin{figure*}[t]
%	\centering
%	\includegraphics[width=0.7\textwidth]{3_inf_LB_UB.png}
%	\caption{Plot comparing our lower bound with numerical evaluations of the upper bound from \cite{Graph_based}, for $d=3$.}
%	\label{fig:3_inf_compare}
%\end{figure*}



Finally, the labelling function, $\mathscr{L}^{(d)}:\mathscr{E}^{(d)}\rightarrow \{0,?,1\}$ is defined as:
\begin{equation}\label{eq:label}
\mathscr{L}^{(d)}(\mathbf{e})=
\begin{cases}
\mathscr{L}^{(d)}_{\text{DB}}(\mathbf{e}), & \text{ if } \mathbf{e}\in \mathscr{E}^{(d)}_{\text{DB}},\\
1, & \text{ if } \mathbf{e}=(\mathbf{q},Q_0) \text{ for } \mathbf{q}\in \mathscr{V}^{(d)}_{\text{DB}},\\
0 & \text{ if } \mathbf{e} = \mathbf{e}^{Q_i}_1 \text{ for some } i\in [0:d-1],\\
? & \text{ if } \mathbf{e} = \mathbf{e}^{Q_i}_2 \text{ for some } i\in [0:d-1].
\end{cases}
\end{equation}

%We note that $\mathscr{G}_Q^{(d)}$ satsifies the properties of a $Q$-graph detailed out in Section \ref{sec:Q-graph}. 
The $Q$-graph, $\mathscr{G}^{(1)}_Q$, is identical to the dynamic programming state diagram under the optimal policy, for the $(1,\infty)$-RLL input-constrained BEC \cite{SabBEC}. The $Q$-graph, $\mathscr{G}^{(2)}_Q$, is shown in Figure \ref{fig:Q_2}.

Our family of $Q$-graphs is then given by $\mathscr{H}:=\{\mathscr{G}^{(d)}_Q: d\in \mathbb{N}\}$, with the $Q$-graph $\mathscr{G}^{({d})}_Q$ being used to derive a lower bound for the $({d},\infty)$-RLL input-constrained BEC.
	
%\begin{remark}
%	The nodes $Q_0, Q_1,\ldots, Q_d$ of $\mathscr{G}^{(d)}_Q$ can be interpreted as follows. Let us define, for a fixed output sequence, $y^t$, the length-$(d+1)$ belief vector $\mathbf{z}_t:=\left(P(S_t=s_t|y^t):s_t\in \mathscr{S}\right)$. Note that the vector,  $\mathbf{z}_t$, which is an element of $\Delta(d)$, is precisely the state vector of the dynamic programming (DP) formulation of the feedback capacity problem \cite{Weiss}. The node $Q_i$ corresponds to the DP state $\mathbf{z}_t = \mathbf{e}_{i}^{d}$, for $i\in [0:d]$. This, in turn, has the interpretation that the nodes $Q_0,\ldots, Q_d$ represent the belief vectors when the decoder knows the channel state exactly.
%	
%%	Now, consider a node $\mathbf{q}\in \mathscr{V}^{(d)}_{\text{DB}}$, where $\mathbf{q}\in \{0,1\}^d$. Let $i_1,\ldots,i_k$, for $k\leq d$, denote the positions of the $?$ entries in in $\mathbf{q}$. We then interpret $\mathbf{q}$ as a proxy for the belief vector, $\mathbf{z}_t$, with non-zero entries in only the co-ordinates $d+1,d+1-i_1,\ldots,d+1-i_k$. Note that by our interpretation, $Q_d$, which represents the $d$-tuple $(0,\ldots,0)\in \mathscr{V}^{(d)}_{\text{DB}}$, corresponds to the belief vector $\mathbf{e}_{d+1}^{d+1}$, as described in the previous paragraph.
%\end{remark}




==> fbcode.tex <==
\label{sec:fbcode}
This section presents a simple feedback coding scheme that achieves the lower bound in Theorem \ref{thm:main}. Our labelling-based coding scheme is similar to the coding schemes in \cite{SabBEC} and \cite{0k}. The main feature of the scheme is a dynamically-changing set of possible messages that is known to both the encoder and the decoder at all times. The objective of the encoder is to communicate a sequence of bits that will enable the decoder to narrow down the set of possible messages to a single message.

Each message $m\in [2^{nR}]$ is mapped uniformly to a point in the unit interval, i.e., the message $m$ is mapped to the point $\frac{m-1}{2^{nR}}$. At each time instant $i$, the unit interval is partitioned into sub-intervals that are labelled by either a `$0$' or a `$1$'. The input $x_i$ to the channel is determined using the label of the sub-interval containing the message. 

The coding scheme proceeds as follows: we first pick positive real numbers $\delta_0,\delta_1,\ldots,\delta_d$ such that $\sum\delta_i\leq 1$. To determine the input bits to be sent, we use a set of $d+2$ labellings, $\mathcal{L}_0,\ldots, \mathcal{L}_d,\hat{\mathcal{L}}$, with the interval $[\sum_{j<i}\delta_j,\sum_{j\leq i}\delta_j)$, in $\mathcal{L}_i$, labelled by a `$1$'. Further, labelling $\hat{\mathcal{L}}$ is such that the entire interval $[0,1)$ is labelled by a `$0$'. Figure \ref{fig:labellings} shows an illustration of the set of labellings.

\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.6\textwidth]{Labellings_new}
	\caption{The set of labellings, $\mathcal{L}_0,\ldots, \mathcal{L}_d$, used in the coding scheme.}
	\label{fig:labellings}
\end{figure}




\begin{algorithm}[t]
	\caption{Coding Scheme}
	\label{alg}
	\begin{algorithmic}[1]		
		\Procedure{Code}{m}       
		\State Set $\mathcal{M}_0 = [2^{nR}]$ and $Y_{1-d}^{0} = (0,\ldots,0)$.
		\State Set Label = $\mathcal{L}_0$.
		\State Set time index $i = 1$.
		\While{$|\mathcal{M}_{i-1}|>1$}
		\State Transmit $X_i = \Gamma(m,\text{Label})$. \Comment{Encoder}
		\If{none of $Y_{i-d}^{i-1}$ is a $1$}
		\If{$Y_i = 0$}
		\State Set $\mathcal{M}_i = \mathcal{M}_{i-1}^{(0)}$.
		\ElsIf{$Y_i=1$}
		\State Set $\mathcal{M}_i =\mathcal{M}_{i-1}^{(1)}$. 
		\Else
		\State Set $\mathcal{M}_i =\mathcal{M}_{i-1}$. 
		\EndIf
		\Else
		\State Set $\mathcal{M}_i =\mathcal{M}_{i-1}$. 
		\EndIf
		\State Label $\leftarrow$ $G(\text{Label},Y_{i-d+1}^{i})$.
		\State Update $i = i+1$.
		\EndWhile
		\State Output $\hat{m}$, where $\mathcal{M}_{i-1} = \{\hat{m}\}$. \Comment{Decoder}
		\EndProcedure
		
	\end{algorithmic}
\end{algorithm} 
The labelling at any time is a function of the channel outputs upto that time instant and can be recursively computed using the previous labelling and previous $d$ channel outputs. Thus, both the encoder and the decoder can compute the labelling used at all times. Let $L_i$ denote the labelling used at time $i$. We fix $L_0 := \mathcal{L}_0$. Then, $L_{i+1} = G(L_i,Y^{i}_{i-d+1})$, where the function $G$ is defined as follows:

\[G(L_i,Y^{i}_{i-d+1}) =
\begin{cases}
	\hat{\mathcal{L}},\ \text{ if one of $Y_{i-d+1}^{i}$ is a 1},\\
	\mathcal{L}_0,\ \text{if $Y_i=0$},\text{ and none} \text{ of $Y_{i-d+1}^{i}$ is a 1},\\
	\mathcal{L}_{\text{$j+1$ mod$(d+1)$}},\ \text{if $L_i = \mathcal{L}_j$, $Y_{i}=?$ and none} \\\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  \text{of $Y_{i-d+1}^{i}$ is a 1}.\\
	%\mathcal{L}_0,\ \text{if $L_i = \hat{\mathcal{L}}$ and none of $Y_{i-d}^{i}$ is a 1.} 
\end{cases}
\]

The transitions between the labellings can be represented by the finite state machine (FSM) shown in Figure \ref{fig:QUB}. The labellings in conjunction with the message are used to determine the bit $X_{i+1}$ to be transmitted. Formally, $X_{i+1} = \Gamma(m,L_{i+1})$, where the function $\Gamma$ is defined as:

\[\Gamma(m,L_{i+1}) =
\begin{cases}
	0,\ \text{if $L_{i+1} = \mathcal{L}_j$, for some $j$, and}\\ \ \ \ \ \ \ \ \ \ \ \ \ \ \text{$\frac{m-1}{2^{nR}} \notin [\sum_{z<j}\delta_z,\sum_{z\leq j}\delta_z)$},\\
	0,\ \text{if $L_{i+1} = \hat{\mathcal{L}}$},\\
	1,\ \text{if $L_{i+1} = \mathcal{L}_j$, for some $j$, and}\\ \ \ \ \ \ \ \ \ \ \ \ \ \ \text{$\frac{m-1}{2^{nR}} \in [\sum_{z<j}\delta_z,\sum_{z\leq j}\delta_z)$}.
\end{cases}
\]
The chronological order of a single use of the channel at time $i$, for a fixed message $m$, thus is $L_i\rightarrow X_i\rightarrow Y_i$, with $L_{i+1} = G(L_i,Y_{i-d+1}^{i})$.

For a given output sequence $y^i$, we denote by $\mathcal{M}_i$ the set of \emph{possible messages} after time $i$, i.e., $\mathcal{M}_i := \{m\in [2^{nR}]: P(m|y^{i})>0\}$, with $\mathcal{M}_0:=[2^{nR}]$. Note that both the encoder and the decoder can compute the conditional distribution $P(m|y^{i})$ using Bayes' rule. We use the notation $\mathcal{M}_i^{(0)}$ and $\mathcal{M}_i^{(1)}$ to denote the set of messages labelled by a `$0$' and by a `$1$', respectively, in $\mathcal{M}_i$.

A transmission at time $i$ is said to be \emph{successful} if $|\mathcal{M}_i|<|\mathcal{M}_{i-1}|$. Specifically, a successful transmission can occur in one of two scenarios: the first is $y_i = 1$, and the second is where $y_i = 0$ and none of $y_{i-d}^{i-1}$ is a $1$. After a successful transmission, the set of possible messages is calculated and expanded uniformly to the unit interval. It is easy to see that in the first kind of successful transmission, the new set of possible messages, $\mathcal{M}_i$, is equal to $\mathcal{M}_{i-1}^{(1)}$, and in the second kind, $\mathcal{M}_i$ equals $\mathcal{M}_{i-1}^{(0)}$. Figure \ref{fig:succ} shows an illustration of the second of the two kinds of successful transmissions. Figure \ref{fig:eras} depicts the situation when a sequence of erasures is received. In this case, the new set of possible messages, $\mathcal{M}_i$, is equal to $\mathcal{M}_{i-1}$. This transmission procedure continues repeatedly until the set of possible messages contains one message. Additionally, we note that the coding scheme is zero-error, since at the end of the algorithm, the decoder can uniquely decode the transmitted message. The encoding and decoding procedures are described in Algorithm \ref{alg}. 
\begin{figure*}[!t]
	\centering
	
	\includegraphics[width=0.7\textwidth]{Q_graph}
	\caption{Figure shows the finite-state machine (FSM) that represents transitions between the labellings, with the edges labelled by outputs. Note that the state of the FSM can be computed at the encoder using the knowledge of the past $d$ outputs alone. When the encoder is in state $Q_i$, for $i\in \{0,1,\ldots,d\}$, the labelling used is $\mathcal{L}_i$, and when the encoder is in state $\hat{Q}_i$, for $i\in \{0,1,\ldots,d\}$, the labelling used is $\hat{\mathcal{L}}$.}
	\label{fig:QUB}
\end{figure*}

The construction of the labellings ensures that the $(d,\infty)$-RLL input constraint is obeyed. This can be seen from the fact that if ever $Y_i = 1$ for some $i$, it holds that the next $d$ inputs are all set to be $0$s. Further, the staggered manner in which the sub-intervals are labelled by a $1$ in the labellings $\mathcal{L}_0,\ldots,\mathcal{L}_d$ ensures that the input constraint is satisfied when a sequence of erasures is received, too. 

The analysis of the rate of the feedback coding scheme is similar to the proofs of Lemma 3 and Lemma 4 in \cite{0k}. In order to make the exposition self-contained, we repeat parts of the proofs here. For a time index $i\in [n]$, we define $\mathsf{J}_i$ to be the number of information bits gained in a single channel use, which is the logarithm of the change in the size of possible messages at the end of the channel use, i.e.,
\begin{equation}
\label{eq:Jk}
\mathsf{J}_i:= \log_2|\mathcal{M}_{i-1}|-\log_2|\mathcal{M}_{i}|.
\end{equation}
 and $\mathsf{L}_i$ to denote the random variable corresponding to the labelling used, with $\mathsf{L}_i\in \mathcal{L} := \{\hat{\mathcal{L}},\mathcal{L}_0,\ldots,\mathcal{L}_d\}$. The following lemma then holds true:

\begin{lemma}
	\label{lem:gain}
	For any time $i\in [n]$, and for all $\ell\in \mathcal{L}$, we have that $\mathbb{E}[\mathsf{J}_i| \mathsf{L}_i=\ell] = \bar{\epsilon}h_b(\delta_\ell)$, where
	\[\delta_\ell = 
	\begin{cases}
		0,\ \text{if $\ell = \hat{\mathcal{L}}$},\\
		\delta_j,\ \text{if $\ell = \mathcal{L}_j$}.
	\end{cases}
	\]
\end{lemma}
\begin{figure}[!t]
	\centering
	
	\includegraphics[width=0.8\textwidth]{Succ1_2}\label{<figure2>}
	\caption{Figure shows an illustration of a successful transmission of the second kind, when $X_1 = Y_1 = 1$, and when the encoder then transmits $d$ additional zeros. Note that the size of the set of possible messages reduces.}
	\label{fig:succ}
\end{figure}

\begin{figure}[!t]
	\centering
%	\subfloat[]{\includegraphics[width=0.5\linewidth]{Succ1_2}\label{fig:succ}}
%	\hfill
%	\subfloat[]{\includegraphics[width=0.5\linewidth]{Eras_4}\label{fig:eras}}
	\includegraphics[width=0.7\textwidth]{Eras_4}
	\caption{The figure shows the setting when two consecutive erasures are received ($Y_1=Y_2=?$), followed by the successful reception of $X_3 = 1$. So long as erasures are received, the set of possible messages is retained as such, while the labellings cycle through $\mathcal{L}_0$ to $\mathcal{L}_d$. Upon the successful reception of $X_3$, the labelling is changed to $\mathcal{L}_0$. However, since the set of possible messages is now a singleton, the transmission ends with the decoder declaring the correct identity of the message.}
	\label{fig:eras}
\end{figure}

\begin{proof}
	We let the random variable $\theta$ denote the indicator that the current output is unerased, i.e.,
	\[
	\theta_i = \mathds{1}\{Y_i\neq `?'\}.
	\]
	Then,
	\begin{align}
		\mathbb{E}[\mathsf{J}_i|\mathsf{L}_i=\ell]&=\epsilon\mathbb{E}[\mathsf{J}_i|\mathsf{L}_i=\ell,\theta_i = 0]+\bar{\epsilon}\mathbb{E}[\mathsf{J}_i|\mathsf{L}_i=\ell,\theta_i = 1] \notag\\
		&= \bar{\epsilon}\mathbb{E}[\mathsf{J}_i|\mathsf{L}_i=\ell,\theta_i = 1] \label{eq:lemm},
	\end{align}
where the second equality holds since if an erasure is received, the set of possible messages remains the same.

We now note that in any of the labellings $\mathcal{L}_j$, it holds that the length of the sub-interval labelled by a `$1$' equals $\delta_j$, and equals $0$ in $\hat{\mathcal{L}}$. Hence, if labelling $\ell \in \mathcal{L}$ is employed, the bit transmitted is distributed according to Ber$(\delta_\ell)$ \footnote{We note as in \cite{0k} that since the messages are discrete points in $[0,1)$, the transmitted bit is actually distributed according to Ber$(\delta_\ell -e_i)$, where $e_i$ is a correction factor that is bounded as $0\leq e_i\leq \frac{1}{|\mathcal{M}_{i-1}|}$. We use Algorithm \ref{alg} for encoding, until a time $t$ such that $|\mathcal{M}_t|\leq 2^{\lambda}$, for an absolute constant, $\lambda>0$. A clean-up coding phase can then be employed, after the labelling-based scheme, similar to \cite[Appendix C]{SabBEC}, using which the remaining at most $\lambda$ bits are then transmitted. The rate of the overall two-stage coding scheme can then be computed to equal the rate calculated using the analysis in this paper.}, where $\delta_\ell$ is as defined in the statement of the theorem.

 Assume that the current size of the set of possible messages, $\mathcal{M}$, equals $k$, with the current labelling used being $\ell$. If the current bit transmitted is received successfully, then, the new set of possible messages has size $k\delta_\ell$, if the current input bit is a `$1$', and is equal to $k\bar{\delta}_\ell$, otherwise. Hence, the expected number of bits required to describe the new set of possible messages is $\bar{\delta}_{\ell} k \log_2(\bar{\delta}_{\ell} k)+\delta_\ell k \log_2(\delta_\ell k) = \log_2(k)-h_b(\delta_{\ell})$. Thus, given that $\mathsf{L}=\ell$, following a successful transmission, the decoder gains $h_b(\delta_{\ell})$ bits of information. Substituting into \eqref{eq:lemm}, we get that
\[
\mathbb{E}[\mathsf{J}|\mathsf{L}=\ell] = \bar{\epsilon}h_b(\delta_\ell).
\]
\end{proof}

The following lemma computes the rate of the proposed coding scheme:
\begin{lemma}
	\label{lem:rate}
	For any $\epsilon \in [0,1]$, the proposed coding scheme achieves a rate
	\[
	R = \max_{\vec{\delta}\in \Delta_d} R(\vec{\delta}),
	\]
	where $R(\vec{\delta})$ is as defined in equation \eqref{eq:R}.
\end{lemma}
\begin{proof}
	Fix $0\leq \delta_0,\delta_1,\ldots,\delta_d\leq 1$, with $\sum_{i=0}^{d}\delta_i \leq 1$. The constraint is chosen so as to ensure that the lengths of the intervals used in the labellings in Figure \ref{fig:labellings} are all non-negative. 
	
	Consider the Markov chain induced by the transitions shown in Figure \ref{fig:QUB}, with the transition probabilities $P(Y=?|q) = \epsilon$, for all $q \in \{Q_0,Q_1,\ldots,Q_d,\hat{Q}_0,\hat{Q}_1,\ldots,\hat{Q}_d\}$, and
	\[
	P(Y=1|q) = 
	\begin{cases}
		\bar{\epsilon}\delta_i, \ \text{if $q = Q_i$, for some $i$},\\
		0, \ \text{otherwise}.
	\end{cases}
	\]
	Let $\pi(\ell)$ denote the stationary probability of using labelling $\ell$, which can be calculated using the stationary probabilities of states of the Markov chain on the FSM. Clearly, for $i\in \{0,1,\ldots,d\}$, $\pi(\mathcal{L}_i)$ equals $\pi(Q_i)$, and $\pi(\hat{\mathcal{L}})$ equals $\sum_{j=0}^{d}\pi(\hat{Q}_j)$. The rate of the coding scheme can be computed to be:
	\begin{align*}
		R &= \lim_{n\rightarrow \infty}  \frac{\log_2 |\mathcal{M}_0|}{n}\\
		&\stackrel{(a)}{=} \lim_{n\rightarrow \infty} \frac{1}{n}\sum_{k=1}^{n}\mathbb{E}[\mathsf{J}_k]\\
		&= \lim_{n\rightarrow \infty}  \frac{1}{n} \sum_{k=1}^{n} \sum_{\ell \in \mathcal{L}} P(\mathsf{L}_k = \ell)\mathbb{E}[\mathsf{J}_k|\mathsf{L}_k = \ell]\\
		&\stackrel{(b)}{=} \sum_{\ell \in \mathcal{L}} \bar{\epsilon}h_b(\delta_\ell) \lim_{n\rightarrow \infty}  \frac{1}{n} \sum_{k=1}^{n} P(\mathsf{L}_k = \ell)\\
		&\stackrel{(c)}{=} \sum_{\ell \in \mathcal{L}} \bar{\epsilon}h_b(\delta_\ell)\pi(\ell)\\
		&= \sum_{i=0}^{d}\bar{\epsilon}h_b(\delta_i)\pi(\mathcal{L}_i)\\
		&\stackrel{(d)}{=} R(\vec{\delta}),
	\end{align*}
where 
\begin{enumerate}[label = (\alph*)]
	\item holds from equation \eqref{eq:Jk},
	\item follows from Lemma \ref{lem:gain} and by exchanging the order of the summations,
	\item follows from the definition of stationary probability and from the fact that the random process $(\mathsf{L}_n:n\in \mathbb{N})$ is a positive recurrent, irreducible, aperiodic Markov chain (this follows from the irreducibility and aperiodicity of the graph in Figure \ref{fig:QUB}), and
	\item holds by an explicit calculation of the stationary probabilities of the Markov process $(\mathsf{L}_n:n\in \mathbb{N})$, which are given by:
	\[
	\pi(\ell)=
	\begin{cases}
		\frac{\epsilon^i}{\sum_{j=0}^{d}\epsilon^j + d\bar{\epsilon}\left(\sum_{j=0}^{d}\epsilon^j\delta_j\right)},\ \ell=\mathcal{L}_i,\\
		\frac{d\bar{\epsilon}\left(\sum_{j=0}^{d}\epsilon^j\delta_j\right)}{\sum_{j=0}^{d}\epsilon^j + d\bar{\epsilon}\left(\sum_{j=0}^{d}\epsilon^j\delta_j\right)},\ \ell=\hat{\mathcal{L}}.
	\end{cases}
	\]
\end{enumerate}
Therefore, maximizing over all allowed parameters $\delta_0,\ldots,\delta_d$, it follows that our coding scheme achieves a rate $R = \max_{\vec{\delta}\in \Delta_d} R(\vec{\delta})$.
\end{proof}

We now provide an upper bound on the feedback capacity of the $(d,\infty)$-RLL input-constrained BEC, using Theorem \ref{thm:UB}.
\begin{lemma}
	\label{lem:ub}
	For any $\epsilon \in [0,1]$, the feedback capacity of the $(d,\infty)$-RLL input-constrained BEC is bounded as:
	\[
	C^{\text{fb}}_{(d,\infty)}\leq \max_{\vec{\delta}\in \Delta_d} R(\vec{\delta}).
	\]
\end{lemma}
\begin{proof}
	We simply apply Theorem \ref{thm:UB} to the $Q$-graph that is the FSM in Figure \ref{fig:QUB}. The transition probabilities $P(Y=y|q)$ are the same as those in the proof of Lemma \ref{lem:rate}, for $y\in \{0,?,1\}$ and $q \in \{Q_0,Q_1,\ldots,Q_d,\hat{Q}_0,\hat{Q}_1,\ldots,\hat{Q}_d\}$. Note that the definition of the transition probabilities implies that 
	\[
	P(X=1|q) = 
	\begin{cases}
		\delta_i, \ \text{if $q = Q_i$, for some $i$},\\
		0, \ \text{otherwise}.
	\end{cases}
	\]
	 We then have that
	 \begin{align*}
	 	I(X;Y|Q) &\stackrel{(a)}{=} H(Y|Q) - H(Y|X)\\
	 	&= H(Y|Q) - h_b(\epsilon)\\
	 	&\stackrel{(b)}{=} \bar{\epsilon}H(X|Q)+h_b(\epsilon) - h_b(\epsilon)\\
	 	&= \sum_{\ell \in \mathcal{L}} \bar{\epsilon}h_b(\delta_\ell)\pi(\ell)\\
	 	&= \sum_{i=0}^{d}\bar{\epsilon}h_b(\delta_i)\pi(\mathcal{L}_i)\\
	 	&= R(\vec{\delta}),
	 \end{align*}
 where
 \begin{enumerate}[label = (\alph*)]
 	\item holds due to the memorylessness of the BEC, and
 	\item follows from the simple identity that $H(a\bar{c},\bar{a}\bar{c},c) = h_b(c)+\bar{c}h_b(a)$, for all $a,c \in [0,1]$.
 \end{enumerate}
Hence, all that remains to be shown for the proof to be complete is that 
\[
\sup_{\{P(x|s,q)\}} R(\vec{\delta}) = \max_{\sum_{i=0}^{d}\delta_i \leq 1}R(\vec{\delta}).
\]
This is true since for any valid input distribution $\{P(x|s,q)\}$ on the $(S,Q)$-graph corresponding to the $Q$-graph in Figure \ref{fig:QUB}, it holds that
\begin{align*}
	\sum_{i=0}^{d}\delta_i = \sum_{i=0}^{d}P(X=1|Q_i)
	&= \sum_{i=0}^{d}\frac{P(X=1,Q_i)}{\pi(\mathcal{L}_i)}\\
	&{=} \sum_{i=0}^{d}\frac{P(X=1,Q_i)}{\epsilon^i \pi(\mathcal{L}_0)}\\
	&= \frac{1}{ \pi(\mathcal{L}_d)}\sum_{i=0}^{d}\epsilon^{d-i}P(X=1,Q_i).	
\end{align*}
Now,
\begin{align*}
    \sum_{i=0}^{d}\delta_i &= \frac{1}{ \pi(\mathcal{L}_d)}\sum_{i=0}^{d}\epsilon^{d-i}P(X=1,Q_i)\\
    &= \frac{1}{ \pi(\mathcal{L}_d)}\sum_{i=0}^{d}\epsilon^{d-i}P(X=1,S=d,Q_i)\\
    &\leq \frac{1}{ \pi(\mathcal{L}_d)}\left(\sum_{i=0}^{d-1}\epsilon^{d-i}P(X=1,S=d,Q_i)+P(S=d,Q_d)\right)\\
    &= \frac{1}{ \pi(\mathcal{L}_d)}\left(\sum_{i=0}^{d-1}P(S=i,Q_d)+P(S=d,Q_d)\right)\\
    &=1,
\end{align*}
where the penultimate equality holds from the structure of the $(S,Q)$-graph.
\end{proof}
\begin{remark}
	We note that for the case when $d=2$, the authors in \cite{0k} provide the optimal $Q$-graph of Figure \ref{fig:QUB} for evaluating an upper bound on the feedback capacity. We have shown here that their upper bound is tight.
\end{remark}
Lemmas \ref{lem:rate} and \ref{lem:ub}, taken together, prove Theorem \ref{thm:main}. We thus obtain an exact characterization of the feedback capacity, in addition to providing an explicit coding scheme.

==> introduction.tex <==

Discrete memoryless channels (DMCs) were introduced by Shannon \cite{Sh48} as models for communication links, and have, since then, been the object of much research activity in information theory. It was shown by Shannon \cite{Sh56} that causal, noiseless feedback of the outputs does not increase the capacity of memoryless channels, which is given by $C = \sup_{P(x)}I(X;Y)$.


In this paper, we consider DMCs with input constraints, which are specific instances of discrete channels with memory, and which find application in magnetic and optical recording systems \cite{Roth}, \cite{Immink}. Such channels fall under the broad category of finite-state channels (or FSCs), the numerical computation of whose non-feedback capacities has been considered in works such as \cite{GBAA} and \cite{Han3}. Figure \ref{fig:genconstdmc} shows a generic DMC with input constraints, with causal, noiseless feedback. The computation of the feedback capacity of an FSC using a dynamic programming (DP) formulation first appeared in \cite{Chen} and was later extended in works such as \cite{Tatikonda1} and \cite{Tatikonda2}. In this work, we shall focus on the binary erasure channel (or BEC), the inputs of which are constrained to obey the $(d,\infty)$-runlength limited (RLL) input constraint\footnote{The $(d,\infty)$-RLL constraint is a special case of the $(d,k)$-RLL constraint on binary sequences, which requires that the length of any run of consecutive $0$s is at least $d$ and at most $k$.}, which mandates that there needs to be at least $d$ $0$s between any pair of successive $1$s. Such RLL input constraints are necessary for mitigating inter-symbol interference and timing and synchronization errors. As was shown in the works \cite{SabBEC}, \cite{Hanerasure}, and \cite{SabBIBO}, the capacities of the $(1,\infty)$-RLL input-constrained binary erasure and binary symmetric channels are strictly larger than their respective non-feedback capacities, for at least some values of the channel parameters, thereby demonstrating that for channels with memory, feedback may indeed increase capacity.

\begin{figure}[!t]
	\centering
	\includegraphics[scale=0.4]{genconstdmc.png}
	\caption{System model of an input-constrained DMC with causal, noiseless feedback.}
	\label{fig:genconstdmc}
\end{figure}

In the context of the BEC with input constraints, the feedback capacities of the $(1,\infty)$- and the $(0,k)$-RLL input constraints (for $k\geq 1$) were computed in the works \cite{SabBEC} and \cite{0k}, respectively. Both of these works put down an explicit coding scheme, whose rate equals the capacity of the BEC with non-causal knowledge of erasures\footnote{Informally, the non-causal capacity is the maximum achievable rate of a coding scheme for the BEC in a setting in which the encoder knows, \emph{prior} to the transmission of the $i^{\text{th}}$ bit $x_i$, whether or not $x_i$ will be erased.}, which, in turn, is as an upper bound on the feedback capacity. Interestingly, this gives rise to the fact that the non-causal capacities of the BEC with the $(1,\infty)$- and the $(0,k)$-RLL input constraints are equal to the respective feedback capacities. Moreover, it was shown in \cite{0k} that the feedback capacity of the $(2,\infty)$-RLL input-constrained BEC is less than the corresponding non-causal capacity, when the channel parameter, $\epsilon$, is equal to $0.5$. In this paper, we show that for the $(2,\infty)$-RLL input-constrained BEC, the feedback capacity is in fact equal to the non-causal capacity for $\epsilon\in [0,1-\frac{1}{2\log(3/2)}]$. This result is a by-product of the main theorem in our paper, which presents an analytical lower bound on the feedback capacity of the $(d,\infty)$-RLL input-constrained BEC, for all $d$ greater than or equal to $1$. For the case when $d=1$, our lower bound is tight for all values of $\epsilon$ \cite{SabBEC}, and for $d=2$, our lower bound is numerically close to an upper bound derived using techniques in \cite{Graph_based}, for $\epsilon$ larger than $1-\frac{1}{2\log(3/2)}$, too. We also present analytical upper bounds on the feedback capacity of the $(d,\infty)$-RLL input-constrained BEC, which, like our lower bounds, are single-parameter optimization problems. We observe that our bounds differ from the non-causal capacity expression (see \cite{0k}) in only the domain of maximization. 

Our techniques involve the use of the single-letter bounding techniques of Sabag et al. in \cite{Single}, and we come up with a specific $Q$-graph (or a $Q$-context mapping) and a choice of a specific ``BCJR-invariant'' input distribution, which gives rise to an achievable rate.

==> preamble.tex <==
% preamble.tex

\geometry{letterpaper, top=2.2in, headheight=1.7in}
\date{}

\makeatletter

\def\fulltitle#1{\def\@fulltitle{#1}}
\def\runningtitle#1{\def\@runningtitle{#1}}
\def\runningauthor#1{\def\@runningauthor{#1}}
\def\affiliation#1{\def\@affiliation{#1}}
\def\department#1{\def\@department{#1}}
\def\memoid#1{\def\@memoid{#1}}
\def\theyear#1{\def\@theyear{#1}}
\def\mydate#1{\def\@mydate{#1}}

\runningtitle{How to write an effective report} % Short title
\author{Your name \and John Doe \and Jane Doe} % Full list of authors
\runningauthor{Your name et al.} % Short list of authors
\affiliation{Your University} % Affiliation e.g. University or Company
\department{Your Department} % Department or Office
\memoid{AI Memo 777} % ID of the tech report
\theyear{2018} % year of the tech report
\mydate{August 08, 2018} %the date

\def\displaymydate{\@mydate}
\def\displaytheyear{\@theyear}
\def\displaymemoid{\@memoid}
\def\displaydepartment{\@department}
\def\displayaffiliation{\@affiliation}
\def\displayrunningauthor{\@runningauthor}
\def\displayrunningtitle{\@runningtitle}

\makeatother

\makeatletter
\patchcmd{\@zfancyhead}{\fancy@reset}{\f@nch@reset}{}{}
\patchcmd{\@set@em@up}{\f@ncyolh}{\f@nch@olh}{}{}
\patchcmd{\@set@em@up}{\f@ncyolh}{\f@nch@olh}{}{}
\patchcmd{\@set@em@up}{\f@ncyorh}{\f@nch@orh}{}{}
\makeatother

% ----------
% fancyhdr setup
% ----------

\pagestyle{fancy}
\renewcommand{\headrulewidth}{0pt}

\fancypagestyle{firstpage}
{
    \fancyhf{}
    \fancyhead{%
        \begin{center}
            \textsc{\displayaffiliation}\\
            \textsc{\displaydepartment}
        \end{center}
        \vspace*{0.5in}
        \displaymemoid
        \hfill
        \displaymydate
    }
    \fancyfoot[L]{\footnotesize \textbf{\textsc{\displayaffiliation} -- \displaytheyear}}
}
\fancyhead[EL]{\small \displayrunningauthor}
\fancyhead[ER]{\small Page \thepage}
\fancyhead[OL]{\small Page \thepage}
\fancyhead[OR]{\small \displayrunningtitle}

\chead{}
\lfoot{}
\cfoot{}
\rfoot{}

% ----------

\providecommand{\keywords}[1]{\noindent \textbf{Keywords:} #1} % keywords definition

\renewcommand{\familydefault}{\sfdefault} % sans-serif font
\setlength{\parskip}{1em} % 1em skip between paragraphs
\abslabeldelim{:} % use colon after the run-in 'Abstract' word
\setlength{\parindent}{0pt} % no indentantion for first page 
\setlength{\abstitleskip}{-\absparindent} % this is because the abstract package sets \absparindent to \parindent

\pretitle{\Large \begin{center}}
\posttitle{\\[2ex] \Large \textbf{by}\end{center}}

==> report_header.tex <==
\usepackage{ifthen}
\usepackage{cite}
\usepackage{algorithm}
\usepackage[cmex10]{amsmath} % Use the [cmex10] option to ensure complicance
% with IEEE Xplore (see bare_conf.tex)
\usepackage{amsthm,amsfonts,amssymb}
\usepackage[noend]{algpseudocode}
\setcounter{MaxMatrixCols}{17}

\usepackage{subfig}
\usepackage{blkarray}
\usepackage[mathscr]{euscript}
\usepackage{enumitem}
%\usepackage{romannum}
\usepackage{blkarray}
\usepackage{stfloats}%
%\newtheorem{theorem}{Theorem}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{lemma}[section]{Lemma}
\theoremstyle{remark}
\newtheorem*{remark}{Remark}
\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
%\theoremstyle{definition}
%\newthorem{definition}{Definition}[section]
%\usetikzlibrary{graphs}
\usepackage{url}
\usepackage{arydshln}
\usepackage{mathtools}
\usepackage{dsfont}
%\usepackage{kbordermatrix}
%\newcommand{\indicator}[1]{\mathbb{1}_{\set{#1}}}
%\usepackage{braket}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor} % Use the [cmex10] option to ensure complicance
% with IEEE Xplore (see bare_conf.tex)

\usepackage{geometry}
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}
\usepackage[runin]{abstract}
\usepackage{titling}
\usepackage{booktabs}
\usepackage{fancyhdr}
\usepackage{helvet}
\usepackage{csquotes}
\usepackage{graphicx}
\usepackage{blindtext}
\usepackage{parskip}
\usepackage{etoolbox}

